Improve Vision Language Model Chain-of-thought Reasoning

Chain-of-thought (CoT) reasoning in vision language models (VLMs) is crucial for improving interpretability and trustworthiness. However, current training recipes lack robust CoT reasoning data, relying on datasets dominated by short annotations with minimal rationales. In this work, we show that training VLM on short answers does not generalize well to reasoning tasks that require more detailed responses. To address this, we propose a two-fold approach. First, we distill rationales from GPT-4o model to enrich the training data and fine-tune VLMs, boosting their CoT performance. Second, we apply reinforcement learning to further calibrate reasoning quality. Specifically, we construct positive (correct) and negative (incorrect) pairs of model-generated reasoning chains, by comparing their predictions with annotated short answers. Using this pairwise data, we apply the Direct Preference Optimization algorithm to refine the model's reasoning abilities. Our experiments demonstrate significant improvements in CoT reasoning on benchmark datasets and better generalization to direct answer prediction as well. This work emphasizes the importance of incorporating detailed rationales in training and leveraging reinforcement learning to strengthen the reasoning capabilities of VLMs.

==> tex/031_evaluation.tex <==
\section{Evaluation of Chain-of-thought Reasoning}
\begin{table}[ht]
\caption{
Evaluation of VLM performance on benchmark datasets with direct and CoT inference.
}
\centering
% \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
    \toprule
    \textbf{Dataset} & \multicolumn{2}{c}{GPT-4o} & \multicolumn{2}{c}{\modelbase} & \multicolumn{2}{c}{\modelformat}  \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    & \textbf{direct} & \textbf{CoT} & \textbf{direct} & \textbf{CoT} & \textbf{direct} & \textbf{CoT} \\
    \midrule
    \aokvqa & 89.61 & 90.13 & 85.87 & 81.22 & - & -  \\
    \chartqa & 79.64 & 84.72 & 68.6 & 41.6 & 70.2 & 70.6 \\
    \docvqa & 90.28 & 90.76 & 74.8 & 50.7 & 75.8 & 64.8  \\
    \infovqa & 72.35 & 72.75 & - & - & 36.23 & 30.77 \\
    \textvqa & 78.1 & 75.43 & 66.1 & 52.3 & 67.8 & 61.1  \\
    \ocrbench & 80.2 & 79.2 & 57.7 & 59.2 & 58.2 & 54.2  \\
    \mathvista & 54.8 & 63.4 & 43.8 & 40.6 & 45.0 & 44.4  \\
    \aitd & 80.67 & 81.48 & 73.0 & 69.9 & 71.4 & 66.9  \\
    \scienceqa & 85.87 & 87.26 & 77.3 & 75.7 & 76.1 & 73.7  \\
    \mmstar & 55.07 & 64.73 & 47.8 & 45.7 & 46.3 & 47.1 \\
    \mmmu & 57.81 & 63.62 & 42.8 & 37.6 & 41.7 & 39.3  \\
    \bottomrule
    \end{tabular}
% }

\label{tab:evaluation_result}
\end{table}


%As shown in \cref{tab:evaluation_result}, the \gpto model demonstrates strong CoT reasoning capabilities, exhibiting superior performance on science reasoning datasets (\mathvista, \aitd, \sqa, \mmmu), chart reasoning (\chartqa), and equal or better performance on \aokvqa, \docvqa, \textvqa, and \ocrbench. For the open-source model, we observed that \modelbase underperforms in direct reasoning tasks, partly due to its tendency to follow prompts too rigidly, leading to errors during answer extraction. However, in the \modelsft setting, our model adheres to the correct format and achieves improved performance on science datasets. Additionally, after reinforcement learning with DPO, we observe better in-domain and out-of-domain generalization.


% \begin{tabularx}{\linewidth}{l|cc|cc}
%     \toprule
%     \textbf{Dataset} & \multicolumn{2}{c}{GPT-4o} & Cambrian & Ours  \\
%     \cmidrule(lr){2-3}
%     & \textbf{direct} & \textbf{CoT} & \textbf{official} & \textbf{best}\\
%     \midrule
%     \aok & 89.6 & 90.1 & 83.1* & 86.2  \\
%     \chartqa & 79.6 & 84.7 & 73.3 & 83.0 \\
%     \docvqa & 90.3 & 90.8 & 77.8 & 82.9   \\
%     \infovqa & 72.4 & 72.8 & 45.7* & 51.6  \\
%     \textvqa & 78.1 & 75.4 & 71.7 & 73.1   \\
%     \aitd & 80.7 & 81.5 & 73.0 & 79.4  \\
%     \sqa & 85.9 & 87.2 & 80.4 & 92.7   \\
%     \mathvista & 54.8 & 63.4 & 49.0 & 50.6  \\
%     \ocrbench & 80.2 & 79.2 & 62.4 &  62.0  \\
%     \mmstar & 55.1 & 64.7 & 50.3* & 54.0  \\
%     \mmmu & 57.8 & 63.6 & 42.7 & 41.6   \\
%     \bottomrule
%     \end{tabularx}
